Asymptotic Analysis of Conditioned Stochastic Gradient Descent

In this paper, we investigate a general class of stochastic gradient descent (SGD) algorithms, called Conditioned SGD, based on a preconditioning of the gradient direction. Using a discrete-time approach with martingale tools, we establish under mild assumptions the weak convergence of the rescaled sequence of iterates for a broad class of conditioning matrices including stochastic first-order and second-order methods. Almost sure convergence results, which may be of independent interest, are also presented. Interestingly, the asymptotic normality result consists in a stochastic equicontinuity property so when the conditioning matrix is an estimate of the inverse Hessian, the algorithm is asymptotically optimal.

==> 3_practical.tex <==

%\section{Practical considerations}

%The aim of this Section is to present and discuss popular optimization schemes used in practice that fall in the framework of \textit{conditioned} stochastic gradient descent.

\section{Practical procedure} \label{sec:application}

For the sake of completeness, the aim of this Section is to derive a feasible procedure that achieves the optimal asymptotic variance described in Corollary \ref{th:convergence_as_final}. First, we present a practical way to compute the \textit{conditioning} matrix $C_k$ and then we show that the resulting algorithm satisfies the high-level conditions of Theorem \ref{th:convergence_weak}. %, namely the almost sure convergence of the iterates $(\theta_k)_{k \geq 0}$ to $\theta^\star$ and of the \textit{conditioning} matrices $(C_k)_{k \geq 0}$ to $H^{-1} $. 
This method is considered in a numerical illustration along with a novel variant of AdaGrad.%Finally, we present a novel variant of AdaGrad which is considered in a numerical experiment.%further details on how to compute stochastic estimates for finite sum optimization.%Finally, to avoid the computational burden of inverting matrices, we also consider a stochastic first-order method with a variant of AdaGrad.

\noindent
\textbf{Construction of the conditioning matrix $C_k$.} %\label{subsec:practical_Ck}
%In virtue of Corollary \ref{th:convergence_as_final}, the limiting matrix $C$ should be close to $H^{-1}$.  
Similarly to the unavailability of gradients, one may not have access to values of the Hessian matrix but only stochastic versions of it (see details in numerical experiments below). As a consequence, we consider the following framework which involves random Hessian matrices. As for gradients,  a policy $(P_k')_{k\geq 0} $ is used at each iteration to produce random Hessians through $H(\theta_{k}, \xi_{k+1}') $ with  $\xi_{k+1}' \sim P_k' $. % We work under the following property.

\begin{assumption}[Unbiased and bounded Hessians]\label{ass:unbiased_hessian}
The Hessian generator $H: \mathbb{R}^{d} \times S \rightarrow \mathbb{R}^{d\times d} $ is uniformly bounded around the minimizer and is such that for all $\theta \in \mathbb R^d$, $H(\theta, \cdot)$ is measurable and we have:\\ $\forall k\geq 0 ,\quad \expect\left[ H (\theta_{k} , \xi_{k+1}')  |\mcf_{k}\right]   =   \nabla^2 F(\theta_{k}).$
 \end{assumption}

\noindent
An estimate of the Hessian matrix $H=\nabla^2 F(\theta^\star)$ is now introduced as the weighted average
\begin{align}\label{weighted_schemes}
\Phi_k =  \sum_{j=0}^k \omega_{j,k}  H (\theta_{j} , \xi_{j+1}') \quad \text{ with } \quad \sum_{j=0}^k \omega_{j,k}  = 1.
\end{align}
The previous estimate has two advantages. First, thanks to averaging, the noise associated to each evaluation $H (\theta_{j} , \xi_{j+1}') $ will eventually vanished due to the sum of martingale increments. Second, the weights  $\omega_{j,k} $ may help to give more importance to most recent iterates. In the idea that $\theta_k $ lies near $\theta^\star$ eventually, it might be helpful to reduce the bias when estimating $H=\nabla^2 F(\theta^\star)$. 

\begin{proposition} \label{prop:cv_ck}
 Let $(\Phi_k)_{k \geq 0}$ be obtained by \eqref{weighted_schemes}.
Suppose that Assumptions  \ref{ass:hessian} and \ref{ass:unbiased_hessian} are fulfilled and that $\theta_k \to \theta^\star$ a.s.  If $\sup_{0 \leq j \leq k}\omega_{j,k} = O(1/k)$,  then we have $\Phi_k \to H = \nabla^2 F(\theta^\star)$ a.s.
\end{proposition}
\noindent
A natural choice is to take equal weights $\omega_{j,k}=(k+1)^{-1}$. However, since  the last iterates are more likely to bring more relevant information through their Hessian estimates, we advocate the use of adaptive weights of the form $\omega_{j,k}  \propto   \exp( -  \eta \| \theta_j - \theta_k\|_1 ) $ with a parameter $\eta \geq 0$ that recovers equal weights with $\eta=0$. These two weights sequences satisfy the assumption of  Proposition \ref{prop:cv_ck}. They are considered in the numerical illustration of the next Section. While inverting $\Phi_k$ would produce a simple estimate of $H^{-1}$, such an approach might result in a certain instability in practice caused by large jumps towards wrong directions (large eigenvalues) or a too restrictive visit along other components (vanishing eigenvalues). 
%In addition, the sequence $(C_k)_{k \geq 0}$ needs to converge to some matrix $C$. 
%Following the result presented in Corollary \ref{th:convergence_as_final}, this limiting matrix $C$ should be close to the inverse of the Hessian $H=\nabla^2 F(\theta^\star)$. One way to satisfy those assumptions is based on the following mixture regularization.
%\smallskip
%\noindent  \textbf{Mixture regularization.}
To overcome this issue, we rely on the following filter which clamps the eigenvalues of a symmetric matrix. For any symmetric matrix $S$ and two positive numbers $0<a<b$, denote by  $S[a,b] $ the associated matrix where all the eigenvalues are clamped to $[a,b]$, \textit{i.e.}, any eigenvalue $\lambda$ of $S$ is modified as $\lambda \leftarrow \max\{a,\min\{\lambda,b\}\}$. 

Let $(\lambda_k^{(m)})_{k\geq 1}$ and $(\lambda_k^{(M)})_{k\geq 1}$ be two sequence of positive numbers such that $\lambda_k^{(m)} \leq \lambda_k^{(M)} $ for all $k\geq 1$. Define the matrices
\begin{align} \label{eq:mixture}
\forall k \in \nset, \quad C_{k} = \left(  \Phi_k [  (\lambda_{k+1}^{(M)})^{-1} , (\lambda_{k+1}^{(m)})^{-1}     ]   \right)^{-1}.
\end{align}
Such a definition guarantees two properties. First,  $C_k \in \mathcal{S}_d^{++}(\rset)$ with $ \lambda_{k+1}^{(m)} I_d \preceq C_k \preceq \lambda_{k+1}^{(M)} I_d$. Second, in virtue of Proposition \ref{prop:cv_ck}, $\Phi_k \to H$ a.s. so that, as soon as $(\lambda_k^{(m)})_{k\geq 1}$ and $(\lambda_k^{(M)})_{k\geq 1}$ go to $0$ and $+\infty$ respectively, the matrix $C_k$ converges almost surely to $H^{-1}$ (as recommended by Corollary \ref{th:convergence_as_final}). Therefore, we obtain a feasible procedure leading to asymptotic optimality. % and this is independent of the general behavior of the sequences  %Note that the parameters $\beta_k$ and $\gamma_k$ are chosen in practice. 



%In particular, the construction proposed in \eqref{eq:mixture} satisfies the assumption of Theorem \ref{th:convergence_as}. As a consequence, we can use Proposition \ref{prop:cv_ck} which leads to the almost sure convergence of $C_k$ to $H^{-1}$. Applying Corollary \ref{th:convergence_as_final} is finally enough to obtain the next statement.

%Note that compared to the conditions of Theorem \ref{th:conv_as_sgd}, only the standard Robbins-Monro condition, Assumption \ref{ass:robbins_monro}, has been replaced by Assumption \ref{ass:robbins_monro_3}. To recover the setting of classical SGD, one can simply choose $C_k = I_d$, in which case, Assumption \ref{ass:robbins_monro_3} meets Assumption \ref{ass:robbins_monro}. This makes Theorem \ref{th:conv_as_sgd} a particular case of our result.

%\subsection{Almost sure convergence of the conditioning matrices $(C_k)$}
%\label{subsec:cvps_matrices}


%For $\theta \in \rset^d$ such that $\|\theta\|_{\infty} \leq 1$, it holds that $\|\theta\|_2^2 \leq \|\theta\|_1$ so the norm may be chosen to promote recent or older Hessian estimates. Adaptive weights of the form $\omega_{j,k} \propto \exp(-\eta \|\theta_j-\theta_k\|_1)$ (resp.  $\omega_{j,k} \propto \exp(-\eta \|\theta_j-\theta_k\|_2^2)$) focus more on recent (resp. past) estimates.


\begin{theorem}[Asymptotic optimality of the iterates] \label{th:optimality_practice} 
Let $(\theta_k)_{k \geq 0}$ be  obtained by conditioned SGD \eqref{eq:cond_sgd} with $\gamma_k = 1/k$, $\Phi_k$ defined by \eqref{weighted_schemes}, $\lambda_k^{(m)} \to 0, \lambda_k^{(M)} \to +\infty$ and $C_k$ given by \eqref{eq:mixture}. Suppose that Assumptions \ref{ass:unbiased} %, \ref{ass:hessian}, \ref{ass:cov}, \ref{ass:lyapunov_bound}, \ref{ass:unbiased_hessian}, \ref{ass:smooth}, \ref{ass:ident}, \ref{ass:exp_smooth}, 
to \ref{ass:robbins_monro_3} are fulfilled and  $\sup_{0 \leq j \leq k}\omega_{j,k} = O(1/k)$.  We have 
\begin{align*}
\sqrt{k} (\theta_k - \theta^\star) \leadsto \mathcal{N}(0, H^{-1} \Gamma H^{-1} ), \qquad \text{as } k\to \infty.
\end{align*}
\end{theorem}
This algorithm is theoretically asymptotically optimal. However in practice, adaptive gradient methods described in Table \ref{table:optimizers} have become the workhorse for training deep learning models as they take advantage of low rank-approximations and diagonal scalings. Interestingly, the \textit{conditioned} matrices involved in these methods are linked to gradient estimates and thus to covariance matrices $\Gamma_k$ (see Assumption \ref{ass:cov}) rather than the Hessian H. Indeed, since $\theta^\star \in \mathcal{S}$, we have for the limiting covariance $\Gamma = \expect_\xi[g(\theta^\star,\xi)g(\theta^\star,\xi)^\top]$. Consider a variant of AdaGrad which accumulates the average gradients $G_k = \delta I + (1/k) \sum_{i=1}^{k} g_i g_i^\top$ and $C_k = G_k^{-1/2}$. Averaging allows to anneal the stochastic noise of the gradient estimate. By the law of large numbers, the limiting matrix in our Theorem \ref{th:convergence_weak} will be $C = (\Gamma + \delta I)^{-1/2}$. For illustrative purposes, this novel method is considered in experiments with futher details in the supplementary material (Appendix \ref{app:numerical}).

\noindent
\textbf{Numerical illustration.} %\label{sec:applis}
Consider the empirical risk minimization framework applied to Generalized Linear Models. Given a data matrix $X=(x_{i,j}) \in \rset^{n \times d}$ with labels $y \in \rset^n$ and a regularization parameter $\lambda>0$, we are interested in  $\min_{\theta \in \rset^d} \{F(\theta)= (1/n) \sum_{i=1}^n f_i(\theta)\}, f_i(\theta)= \mathcal{L}(x_i^\top \theta,y_i) + \lambda \Omega(\theta),$ % the following optimization problem where 
%\begin{align*}
%F(\theta) = \frac{1}{n} \sum_{i=1}^n f_i(\theta), \quad  f_i(\theta)= \mathcal{L}(x_i^\top \theta,y_i) + \lambda \Omega(\theta),
%\end{align*}
$\mathcal{L}:\rset \times \rset \to \rset$ is smooth loss function and $\Omega: \rset^d \to \rset_+$ is a smooth convex regularizer chosen as Tikhonov regularization $\Omega(\theta) = \frac{1}{2}\|\theta\|_2^2$. The gradient and Hessian of each component $f_i$ are given by $\nabla f_i(\theta) = \mathcal{L}'(x_i^\top \theta,y_i)x_i + \lambda \theta, \nabla^2 f_i(\theta) = \mathcal{L}''(x_i^\top \theta,y_i)x_i x_i^\top + \lambda I_d$ where $\mathcal{L}'(\cdot,\cdot)$ and $\mathcal{L}''(\cdot,\cdot)$ are the first and second derivative of $\mathcal{L}(\cdot,\cdot)$ with respect to the first argument. %Consider two well-known losses, namely least-squares and logistic. These losses are respectively associated to the Ridge regression problem with $y \in \rset^n$ and the binary classication task with $y \in \{-1,+1\}^n$. %The regularization parameter is set to the classical value $\lambda=1/n$. 
%Denote by $\sigma(z) = 1/(1+\exp(-z))$ the sigmoid function, we have the following closed-form equations for the Ridge regression
%\begin{align*}
%\mathcal{L}(x_i^\top \theta,y_i) &=  (y_i - x_i^\top \theta)^2 / 2 \\
%(Ridge) \quad \mathcal{L}'(x_i^\top \theta,y_i) &= x_i^\top \theta - y_i \\
%\mathcal{L}''(x_i^\top \theta,y_i) &=1
%\end{align*} 
%and for the logistic regression
%\begin{align*}
%\mathcal{L}(x_i^\top \theta,y_i) &= \log(1+\exp(-y_i x_i^\top \theta)) \\
%(Logistic) \quad \mathcal{L}'(x_i^\top \theta,y_i) &= \sigma(x_i^\top \theta)-y_i \\
%\mathcal{L}''(x_i^\top \theta,y_i) &= \sigma(x_i^\top \theta)(1-\sigma(x_i^\top \theta)).
%\end{align*}
 As stated in Example 1 of Section \ref{sec:csgd_math_background}, stochastic versions of both the gradient and the Hessian of the objective $F$ can be easily computed using only a batch $B \subset \{ 1,\ldots,n \}$ of data and $\nabla_B F(\theta) = \sum_{i \in B} \nabla f_i(\theta)/|B|$ (resp. $\nabla_B^2 F(\theta) = \sum_{i \in B} \nabla^2 f_i(\theta)/|B|$) for the gradient (resp. Hessian) estimate. Note that these random generators meet Assumptions \ref{ass:unbiased} and \ref{ass:unbiased_hessian} as they produce unbiased estimates of the gradient and the Hessian matrix respectively. 
 
\noindent
We focus on Ridge regression on simulated data with $n = 10,000$ samples in dimensions $d \in \{20; 100\}$ and \textit{Boston Housing dataset} \citep{harrison1978hedonic} ($n=506;d=14$) with $|B|=16$. Starting from $\theta_0=(0,\ldots,0) \in \rset^d$, we use optimal learning rate of the form $\gamma_k = \alpha/(k+k_0)$ \citep{bottou2018optimization} and set $\lambda_k^{(m)} \equiv 0, \lambda_k^{(M)} = \Lambda \sqrt{k}$ where $\alpha,k_0$ and $\Lambda$ are tuned using a grid search. The means of the optimality ratio $k \mapsto [F(\theta_k)-F(\theta^\star)]/[F(\theta_0)-F(\theta^\star)]$, obtained over $100$ independent runs, are presented in Figure \ref{fig:simulated}. The methods in competition are \textit{sgd}: standard SGD; \textit{sgd\_avg}: Polyak-averaging variant with a burn-in period; \textit{csgd}($\eta=0$) and \textit{csgd}($\eta>0$): \textit{conditioned} sgd methods with equal and adaptive weights where the matrix $\Phi_k$ is given by Eq. \eqref{weighted_schemes}; \textit{adafull\_avg}: the variant of Adagrad presented above with an average for $G_k$.% instead of the cumulative sum provided in the literature of Adagrad. 
 
  \begin{figure}[h!]
  \centering
  \subfigure[Ridge $d=20$]{
  \includegraphics[scale=0.33]{graph/ridge_n10000_d20.pdf}\label{fig:ridged20}}
  \subfigure[Ridge $d=100$]{
  \includegraphics[scale=0.33]{graph/ridge_n10000_d100.pdf}\label{fig:ridged100}}
  \subfigure[Boston Dataset]{
  \includegraphics[scale=0.33]{graph/ridge_boston.pdf}\label{fig:boston}}
    \caption{$k \mapsto [F(\theta_k)-F(\theta^\star)]/[F(\theta_0)-F(\theta^\star)]$ on synthetic data (a-b) and Boston dataset (c).}
    \label{fig:simulated}
\end{figure}
\vspace{-1cm}

==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

